Security of Electrical, Optical and Wireless On-Chip Interconnects: A Survey

The advancement of manufacturing technologies has enabled the integration of more intellectual property (IP) cores on the same system-on-chip (SoC). Scalable and high throughput on-chip communication architecture has become a vital component in today's SoCs. Diverse technologies such as electrical, wireless, optical, and hybrid are available for on-chip communication with different architectures supporting them. Security of the on-chip communication is crucial because exploiting any vulnerability would be a goldmine for an attacker. In this survey, we provide a comprehensive review of threat models, attacks, and countermeasures over diverse on-chip communication technologies as well as sophisticated architectures.

==> sections/TBD.tex <==
\section{TBD}

Lack of insights: The survey fails to provide insights and interesting take-away messages from the study. I would suggest that the authors clearly underscore the key insights from the study by providing takeaway messages and guidelines on security-aware NoC design. Adding a section after Section 5 and summarizing the study by providing guidelines is essential.

Key takeaways for security aware NoC Design.

\begin{itemize}
    \item Having hybrid NoC architectures with two/more (electrical/wireless/op) the security of NoC should support multitude of attacks. (Countermeasures effective across multiple technologies.)
    \item Complex security attacks using machine learning. 
    \item Offline security attacks and countermeasures (Adversaries have unlimited resources, can do differential/ cryptanalysis elsewhere with more computing power)
    \item Balancing between Security vs Performance (Prioritize what security concepts are critical, strong/weak security models and act accordingly)
    \item Simple and architecture specific security countermeasures. (Traditional or variants of them than what use underline architectural features are much suitable because of low ovrhead power and area.)
    \item Application Specific NoC and Security.( Accelerators multicast, GPU supporting dataflows. SoC vs GPU NoCs)
    \item Side channel attacks on new technologies.
\end{itemize}


NoC is the core component responsible for communication in SoCs with large number of tiles. In this paper, we perform a comprehensive survey about attacks, threat models and countermeasures of diverse on-chip communication technologies (electrical, optical, wireless, and hybrid) and architectures. .







